Modelling Political Coalition Negotiations Using LLM-based Agents

Coalition negotiations are a cornerstone of parliamentary democracies, characterised by complex interactions and strategic communications among political parties. Despite its significance, the modelling of these negotiations has remained unexplored with the domain of Natural Language Processing (NLP), mostly due to lack of proper data. In this paper, we introduce coalition negotiations as a novel NLP task, and model it as a negotiation between large language model-based agents. We introduce a multilingual dataset, POLCA, comprising manifestos of European political parties and coalition agreements over a number of elections in these countries. This dataset addresses the challenge of the current scope limitations in political negotiation modelling by providing a diverse, real-world basis for simulation. Additionally, we propose a hierarchical Markov decision process designed to simulate the process of coalition negotiation between political parties and predict the outcomes. We evaluate the performance of state-of-the-art large language models (LLMs) as agents in handling coalition negotiations, offering insights into their capabilities and paving the way for future advancements in political modelling.

==> tables/main_results.tex <==
\begin{figure*}[!ht]
    \label{figure:main}
    \centering
    % Row 1
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tikzpicture}
            \begin{axis}[
                title = Austria 2013,
                xbar, % Use xbar for horizontal bars
                enlargelimits=0.15,
                legend style={at={(0.5,-0.10)},
                  anchor=north,legend columns=1},
                xlabel={Value},
                symbolic y coords={llama-7b-chat,llama-13b-chat,GPT-3.5},
                ytick=data,
                nodes near coords,
                nodes near coords align={horizontal},
                bar width=10pt,
                enlarge y limits = 0.4,
                fill,
                %bar shift=0pt,
                ]
            
            % Social Democratic Party
            
            % Austrian Poeple's Party
            
            
            \legend{Social Democratic Party, Austrian Poeple's Party}
            \end{axis}
        \end{tikzpicture}}
        %\caption{Chart A}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tikzpicture}
            \begin{axis}[
                title = Germany 2013,
                xbar, % Use xbar for horizontal bars
                enlargelimits=0.15,
                legend style={at={(0.5,-0.10)},
                  anchor=north,legend columns=1},
                xlabel={Value},
                symbolic y coords={llama-7b-chat,llama-13b-chat,GPT-3.5},
                ytick=data,
                nodes near coords,
                nodes near coords align={horizontal},
                bar width=10pt,
                enlarge y limits = 0.4,
                fill,
                %bar shift=0pt,
                ]
            
            %  Christian Democratic Union
            
            % Social Democratic Party
            
            \legend{Christian Democratic Union, Social Democratic Party}
            \end{axis}
        \end{tikzpicture}}
        %\caption{Chart B}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tikzpicture}
            \begin{axis}[
                title = Iceland 2013,
                xbar, % Use xbar for horizontal bars
                enlargelimits=0.15,
                legend style={at={(0.5,-0.10)},
                  anchor=north,legend columns=1},
                xlabel={Value},
                symbolic y coords={llama-7b-chat,llama-13b-chat,GPT-3.5},
                ytick=data,
                nodes near coords,
                nodes near coords align={horizontal},
                bar width=10pt,
                enlarge y limits = 0.4,
                fill,
                %bar shift=0pt,
                ]
            
            %  Independence Party
            
            %  Progressive Party
            
            
            \legend{Independence Party,Progressive Party}
            \end{axis}
        \end{tikzpicture}}
        %\caption{Chart C}
    \end{subfigure}

    % Row 2
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tikzpicture}
            \begin{axis}[
                title = Ireland 2011,
                xbar, % Use xbar for horizontal bars
                enlargelimits=0.15,
                legend style={at={(0.5,-0.10)},
                  anchor=north,legend columns=1},
                xlabel={Value},
                symbolic y coords={llama-7b-chat,llama-13b-chat,GPT-3.5},
                ytick=data,
                nodes near coords,
                nodes near coords align={horizontal},
                bar width=10pt,
                enlarge y limits = 0.4,
                fill,
                %bar shift=0pt,
                ]
            
            % Fine Gael 
            
            % Labour Party
            
            
            \legend{Fine Gael, Labour Party}
            \end{axis}
        \end{tikzpicture}}
        %\caption{Chart D}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tikzpicture}
            \begin{axis}[
                title = Netherlands 2012,
                xbar, % Use xbar for horizontal bars
                enlargelimits=0.15,
                legend style={at={(0.5,-0.10)},
                  anchor=north,legend columns=1},
                xlabel={Value},
                symbolic y coords={llama-7b-chat,llama-13b-chat,GPT-3.5},
                ytick=data,
                nodes near coords,
                nodes near coords align={horizontal},
                bar width=10pt,
                enlarge y limits = 0.4,
                fill,
                %bar shift=0pt,
                ]
            
            %  People's Party for Freedom and Democracy 
            
            % Labour Party
            
            
            \legend{ People's Party for Freedom and Democracy, Labour Party}
            \end{axis}
        \end{tikzpicture}}
        %\caption{Chart E}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tikzpicture}
            \begin{axis}[
                title = Portugal 2011,
                xbar, % Use xbar for horizontal bars
                enlargelimits=0.15,
                legend style={at={(0.5,-0.10)},
                  anchor=north,legend columns=1},
                xlabel={Value},
                symbolic y coords={llama-7b-chat,llama-13b-chat,GPT-3.5},
                ytick=data,
                nodes near coords,
                nodes near coords align={horizontal},
                bar width=10pt,
                enlarge y limits = 0.4,
                fill,
                %bar shift=0pt,
                ]
            
            %  Social Democratic Party
            
            % CDS – People's Party
            
            
            \legend{ Social Democratic Party, CDS – People's Party}
            \end{axis}
        \end{tikzpicture}}
        %\caption{Chart F}
    \end{subfigure}
    \caption{Composite Figure of Six Bar Charts}
\end{figure*}




==> tables/simulation.tex <==
\begin{table*}[]
    \centering
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{l}
         \hline
         Algorithm: Policy-Based Negotiation \\ 
         \hline
         Input: \A, \B, List of Policies \\
         Output: Agreements on Policies \\
         \texttt{1. Initialise agents (\A and \B).} \\
         \texttt{2. Initialise the list of policies to be negotiated.}\\
         \texttt{3. While there are policies in the list:}\\
            \hspace{10mm}\texttt{a. Select the next policy, current policy.}\\
            \hspace{10mm}\texttt{b. \A proposes current policy to \B along with an explanatory rationale.}\\
            \hspace{10mm}\texttt{c. \B evaluates current policy based on the rationale and internal criteria.}\\
            \hspace{10mm}\texttt{d. If \B decides to SUPPORT current policy:}\\
                \hspace{20mm}\texttt{i. An agreement on current policy is reached.}\\
                \hspace{20mm}\texttt{ii. Record the agreement.}\\
            \hspace{10mm}\texttt{e. If \B decides to OPPOSE current policy:}\\
                \hspace{20mm}\texttt{i. \A chooses an action, action  {SUPPORT, DROP, REFINE, COMPROMISE}.}\\
                \hspace{20mm}\texttt{ii. If action is SUPPORT:}\\
                    \hspace{30mm}\texttt{- No changes}\\
                \hspace{20mm}\texttt{iii. If action is DROP:}\\
                    \hspace{30mm}\texttt{- Discard current policy.}\\
                \hspace{20mm}\texttt{iv. If action is REFINE:}\\
                    \hspace{30mm}\texttt{- \A proposes a refined version of current policy.}\\
                \hspace{20mm}\texttt{v. If action is COMPROMISE:}\\
                    \hspace{30mm}\texttt{- \A selects a compromise policy from its proposals.}\\
                    \hspace{30mm}\texttt{- If \B accepts the compromise:}\\
                        \hspace{40mm}\texttt{- An agreement on current policy is reached.}\\
                        \hspace{40mm}\texttt{- Record the agreement.}\\
            \hspace{10mm} \texttt{f. Move to the next policy in the list.}\\
         \texttt{4. End of negotiation.}\\
         \texttt{5. Output the recorded agreements.}\\
         \hline
    \end{tabular}}
    %\caption{Caption}
    \label{tab:negotitation}
\end{table*}
